Protect Your Secrets: Understanding and Measuring Data Exposure in VSCode Extensions

Recent years have witnessed the emerging trend of extensions in modern Integrated Development Environments (IDEs) like Visual Studio Code (VSCode) that significantly enhance developer productivity. Especially, popular AI coding assistants like GitHub Copilot and Tabnine provide conveniences like automated code completion and debugging. While these extensions offer numerous benefits, they may introduce privacy and security concerns to software developers. However, there is no existing work that systematically analyzes the security and privacy concerns, including the risks of data exposure in VSCode extensions. In this paper, we investigate on the security issues of cross-extension interactions in VSCode and shed light on the vulnerabilities caused by data exposure among different extensions. Our study uncovers high-impact security flaws that could allow adversaries to stealthily acquire or manipulate credential-related data (e.g., passwords, API keys, access tokens) from other extensions if not properly handled by extension vendors. To measure their prevalence, we design a novel automated risk detection framework that leverages program analysis and natural language processing techniques to automatically identify potential risks in VSCode extensions. By applying our tool to 27,261 real-world VSCode extensions, we discover that 8.5% of them (i.e., 2,325 extensions) are exposed to credential-related data leakage through various vectors, such as commands, user input, and configurations. Our study sheds light on the security challenges and flaws of the extension-in-IDE paradigm and provides suggestions and recommendations for improving the security of VSCode extensions and mitigating the risks of data exposure.

==> sections/threats.tex <==
\section{Threats to Validity}
\label{sec:threats}

Below, we discuss threats that may impact the results of our study.

\textbf{Threats to the external validity}
xxxxx



\textbf{Threats to the internal validity}
xxxxx

\textbf{Threats to the construct validity}
xxxxxxx


==> tables/tab2_performance_compare.tex <==
% Table generated by Excel2LaTeX from sheet 'acc'
\begin{table}[t]
  \centering
  \caption{Approach Comparison}
  \scalebox{0.85}{
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{Classifier} & \textbf{Accuracy} & \textbf{F1} & \textbf{TPR} & \textbf{TNR} \\
    \midrule
    \textbf{BERT} & 99.59\% & 99.59\% & 93.02\% & 99.76\% \\
    \textbf{ChatGPT-S} & 97.25\% & 44.07\% & 41.44\% & 98.75\% \\
    \textbf{ChatGPT-L} & 98.08\% & 44.44\% & 29.28\% & 99.93\% \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:2performance_compare}%
\end{table}%

